Wrapping nonspherical vesicles at bio-membranes

The wrapping of particles and vesicles by lipid bilayer membranes is a fundamental process in cellular transport and targeted drug delivery. Here, we investigate the wrapping behavior of nonspherical vesicles, such as ellipsoidal, prolate, oblate, and stomatocytes, by systematically varying the bending rigidity of the vesicle membrane and the tension of the planar membrane. Using the Helfrich Hamiltonian, triangulated membrane models, and energy minimization techniques, we predict multiple stable wrapping states and identify the conditions for their coexistence. Our results demonstrate that softer vesicles bind more easily to planar membranes; however, achieving complete wrapping requires significantly higher adhesion strengths compared to rigid particles. As membrane tension increases, deep-wrapped states disappear at a triple point where shallow-wrapped, deep-wrapped, and complete-wrapped states coexist. The coordinates of the triple point are highly sensitive to the vesicle shape and stiffness. For stomatocytes, increasing stiffness shifts the triple point to higher adhesion strengths and membrane tensions, while for oblates it shifts to lower values, influenced by shape changes during wrapping. Oblate shapes are preferred in shallow-wrapped states and stomatocytes in deep-wrapped states. In contrast to hard particles, where optimal adhesion strength for complete wrapping occurs at tensionless membranes, complete wrapping of soft vesicles requires finite membrane tension for optimal adhesion strength. These findings provide new insights into the interplay between vesicle deformability, shape, and membrane properties, advancing our understanding of endocytosis and the design of advanced biomimetic delivery systems.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
